M-QALM: A Benchmark to Assess Clinical Reading Comprehension and Knowledge Recall in Large Language Models via Question Answering

There is vivid research on adapting Large Language Models (LLMs) to perform a variety of tasks in high-stakes domains such as healthcare. Despite their popularity, there is a lack of understanding of the extent and contributing factors that allow LLMs to recall relevant knowledge and combine it with presented information in the clinical and biomedical domain: a fundamental pre-requisite for success on down-stream tasks. Addressing this gap, we use Multiple Choice and Abstractive Question Answering to conduct a large-scale empirical study on 22 datasets in three generalist and three specialist biomedical sub-domains. Our multifaceted analysis of the performance of 15 LLMs, further broken down by sub-domain, source of knowledge and model architecture, uncovers success factors such as instruction tuning that lead to improved recall and comprehension. We further show that while recently proposed domain-adapted models may lack adequate knowledge, directly fine-tuning on our collected medical knowledge datasets shows encouraging results, even generalising to unseen specialist sub-domains. We complement the quantitative results with a skill-oriented manual error analysis, which reveals a significant gap between the models' capabilities to simply recall necessary knowledge and to integrate it with the presented context. To foster research and collaboration in this field we share M-QALM, our resources, standardised methodology, and evaluation results, with the research community to facilitate further advancements in clinical knowledge representation learning within language models.

==> section/datasets.tex <==
\section{Datasets}

Our proposed benchmark builds upon MultiMedQA by expanding in several key areas. Firstly, we aim to test the models' reading comprehension capabilities rigorously. Secondly, we broaden the scope to include questions from specialized medical domains and geographic locales. Lastly, we incorporate more datasets that test context-based reasoning into the evaluation. Our benchmark comprises 22 datasets, including traditional MCQs, context-based MCQs, and abstractive question-answering datasets. 

\subsection{Datasets Utilized}


\begin{enumerate}
    \item \textbf{USMLE - English}: We employ the USMLE dataset obtained from the MedQA paper \cite{medqa}, comprising questions from the Medical Licensing Exam conducted in the US. We retain this dataset's original training, validation, and test set divisions.
    
    \item \textbf{MEDMCQA}: We incorporate the MEDMCQA dataset from \cite{medmcqa}, which comprises medical questions from Indian Medical Entrance Exams. We retain this dataset's original training, validation, and test set splits. Similar to \cite{medpalm1}, we evaluate all models on the validation set since we lack access to the test set ground truth.

    \item \textbf{MMLU}: Following the design of \cite{medpalm1}, we incorporate a subset of the MMLU datasets \cite{mmlu} specifically curated to assess medical domain knowledge. 

    \item \textbf{MEDIQA-ANS}: The MEDIQA 2019 shared task introduced the MEDIQA-QA dataset \cite{mediqa-ans} for answer-ranking, comprising consumer health questions and passages from reputable online sources. The dataset was curated by extracting passages from the text of web pages, and it includes manually generated single and multi-document summaries in both extractive and abstractive forms. We employ the multi-document abstractive summary as the ground truth reference answer for our questions. We specifically filter for questions and answers marked as excellent. We utilize this solely for evaluating models.
    
    \item \textbf{HEADQA}: We include the HEADQA dataset \cite{headqa}, which comprises graduate-level questions (MCQs) about various fields of medicine used for examinations to apply for specialization positions in the Spanish public healthcare system. We use the English version of the dataset and retain the original train, validation, and test split. 

    \item  \textbf{PubmedQA}: The PubMedQA dataset \cite{pubmedqa} is a biomedical question-answering dataset comprising 1,000 expert-annotated QA instances. Each instance necessitates reasoning over a PubMed abstract to answer a relevant question. While the dataset provides both long and short answers (yes, no, or maybe), we focus exclusively on the short answers for our evaluation, thereby generalizing the task as MCQ evaluation. We retain the original test split of 500 questions. Additionally, we allocate 100 questions from the training set to serve as a validation set, facilitating standardized training and validation in future studies.

    \item \textbf{BioMRC}: The BioMRC dataset \cite{biomrc} focuses on machine reading comprehension within the biomedical domain. It is structured in a cloze-style format, where questions are based on biomedical abstracts where biomedical entities are replaced with "pseudo-identifiers". The task is to identify these masked entities from a set of options. We utilize two compact versions of BioMRC: tiny A and tiny B, each corresponding to different settings, A and B, respectively. In Setting A, also known as tiny A, pseudo-identifiers are consistent across the dataset. This design allows models to learn about the entities from their multiple occurrences. On the other hand, Setting B, or tiny B, resets the pseudo-identifiers for each question, requiring models to answer based solely on the given passage and question. We retain the original structure of Setting B. However, evaluating Setting A becomes challenging in our context, as we do not use the BioMRC training corpus. To address this limitation, we modify Setting A to include the original entity names and their corresponding pseudo-identifiers in the answer options. This aims to assess whether the model can accurately answer when provided with the original entity names.
     
    \item \textbf{Processbank}: The Processbank dataset \cite{processbank} is designed for machine reading comprehension, featuring questions based on paragraphs describing biological processes. Each question, associated with a particular paragraph, has two answer options. The dataset comes with a predefined split of 435 questions (150 files) for training and 100 questions (50 files) for testing. We allocate 25 files from the training set to create a validation set while retaining the original test set for model evaluation.

    
    \item \textbf{QA4MRE - Alzheimer's disease QA}: The dataset proposed by \citet{qa4mre} contains MCQ questions regarding Alzheimer's disease, aimed at assessing machine reading systems' ability to answer questions about the disease by parsing relevant documents. We have adapted this dataset to an open-ended MCQ task to evaluate LLMs' ability to answer these questions based on inherent knowledge. This dataset is employed solely for model evaluation purposes.
    
    
    \item \textbf{BioASQ}: The BioASQ dataset \cite{bioasq1} \cite{bioasq2} features biomedical questions crafted by experts. We utilize the BioASQ 2022 dataset \cite{bioasq1} \cite{bioasq2} to prepare our dataset. The BioASQ dataset is divided into two parts: one for multiple choice questions (MCQs) and another for long-form question answering (QA).For the MCQ part, we filter out the yes/no questions from BioASQ, converting them into an MCQ format to create a new subset, which we term \textbf{BioASQ-MCQ}. We manually create a training-validation (train-val) split of roughly 85\%-15\% from the filtered questions, resulting in 975 training questions, 173 validation questions and retaining a test set of 123 questions. For the long-form QA part, BioASQ provides fact, list, and bullet-type questions. We compile these into a long-form QA dataset, ensuring a balanced representation of all question types in training and validation sets. The train-validation split results in 4733 training and 697 validation questions, with approximately 15\% of all question types in the validation set.

    \item \textbf{MASH-QA:} The MASH-QA dataset \citet{mashqa} was designed for answering medical questions based on paragraphs where answers may span multiple text segments. Initially intended for extractive answering tasks, we repurpose it as an abstractive QA task, utilizing the extractive answers as the reference ground truth.

    \item \textbf{MedQUAD:}
    The MedQUAD dataset \cite{medquad} encompasses medical question-answer pairs extracted from various National Institute of Health (NIH) websites, covering topics on diseases, drugs, and other medical entities. Only nine of the twelve websites contributing to the original dataset have answers. We segregate questions from these nine websites and devise a train-validation (train-val) split, assigning data from six websites for training and data from the remaining three websites for validation.

    \item \textbf{TREC-2017 LiveQA}:
    We employ the TREC-2017 LiveQA dataset \cite{liveqa} for evaluation purposes. Specifically, we leverage the rankings provided within the MedQUAD evaluation process \cite{medquad} to keep question-answer pairs that have answer rating as excellent.

    \item \textbf{British Ophthalmology Practice Tests}: We employ sample questions from the Fellowship of the Royal College of Ophthalmologists (FRCOphth) exams, as provided by the Royal College of Ophthalmologists on their website\footnote{\url{https://www.rcophth.ac.uk/wp-content/uploads/2022/01/Part-1-FRCOphth-Sample-MCQs.pdf}}\footnote{\url{https://www.rcophth.ac.uk/wp-content/uploads/2022/01/Part-2-FRCOphth-Written-Sample-MCQs-20160524.pdf}}~\cite{opth}. These \mcqa{} questions, geared towards testing ophthalmology-related knowledge, are used for evaluation.
    
    \item \textbf{MEDINFO}:
    The MEDINFO dataset, introduced by \citet{medinfo}, consists of real consumer questions concerning medications and drugs. It encompasses 674 question-answer pairs, which we employ solely for evaluation purposes.
    \end{enumerate}
